Supporting Multi-point Fan Design with Dimension Reduction

Motivated by the idea of turbomachinery active subspace performance maps, this paper studies dimension reduction in turbomachinery 3D CFD simulations. First, we show that these subspaces exist across different blades---under the same parametrization---largely independent of their Mach number or Reynolds number. This is demonstrated via a numerical study on three different blades. Then, in an attempt to reduce the computational cost of identifying a suitable dimension reducing subspace, we examine statistical sufficient dimension reduction methods, including sliced inverse regression, sliced average variance estimation, principal Hessian directions and contour regression. Unsatisfied by these results, we evaluate a new idea based on polynomial variable projection---a non-linear least squares problem. Our results using polynomial variable projection clearly demonstrate that one can accurately identify dimension reducing subspaces for turbomachinery functionals at a fraction of the cost associated with prior methods. We apply these subspaces to the problem of comparing design configurations across different flight points on a working line of a fan blade. We demonstrate how designs that offer a healthy compromise between performance at cruise and sea-level conditions can be easily found by visually inspecting their subspaces.

==> sec-1a.tex <==
\section{Introduction and motivation}
\label{sec:intro}
It is virtually impossible today for a computational simulation to replicate the unsteady, complex, and random nature of fluid moving through an engine at cruise; there are simply far too many unknowns. Blades in a single row are susceptible to manufacturing variations, the casing is never perfectly circular, operating conditions exhibit some variability, and state-of-the-art 3D unsteady solvers model the turbulence and do not resolve all the pertinent scales and their evolution. Our best window into this world is undoubtedly the data that arises from engine tests.

The challenge with engine tests is that they typically have low instrumentation coverage as there is limited space for instrumentation and capacity for acquiring signals from the various measurement devices. Furthermore, access to specific areas of interest in the gas path is extremely limited. In a rig, by contrast, the temperatures, pressures and vibration levels will generally be reduced, though they do offer greater access for instrumentation. The measurement methods in a rig may also be different from those in an engine, i.e., certain probe designs that are not permissible in an engine may be used in a rig. That said, the rig is never fully representative of the engine, in particular, it does not fully capture the interactions between adjacent components in the engine. 

Our focus in this paper will be on on-ground engine temperature measurements, obtained from a series of rakes at a specific axial station. We wish to study these temperature values, as they cannot be reproduced in rigs or CFD. Consider the schematic shown in Figure~\ref{fig:measurements}. One can consider the spatial variation of engine temperature to be a superposition of engine modes (not visible in a rig), blade-to-blade modes (likely visible in a rig), and noise. The blade-to-blade modes originating from leakage flows, tip vortices, stator and rotor wakes and upstream potential fields lie at the higher end of the frequency spectrum (see page 9 of \cite{ernst2011analysis}) as these will be functions of the blade numbers. They can be experimentally determined using time resolved temperature and pressure traverse measurements. Annular asymmetries in these measurements are expected as a superposition of blade-to-blade modes with the engine modes will result in variations in viscous mixing effects, inviscid wake stretching and the transport of low momentum wake air across the passage \cite{sanders2002multi, mailach2008periodical}. Engine modes, by contrast, are captured by positioning rakes at the same pitch relative to the upstream stator vanes. Asymmetries in engine modes can be introduced by upstream bleed positions, upstream ducts, structural members and downstream potential fields. 

So what is typically done with engine measurements? The first notion is to arithmetically average them. In fact, historically, engines were fitted with equal area weighted probes (see \cite{stoll1979effect, francis1989measurement}) permitting relatively straightforward area average calculations. Over the years different averaging techniques have emerged (see Cumpsty and Horlock \cite{cumpsty2006averaging} for a thorough review) including the work-average method of Pianko \cite{pianko1983propulsion}, the momentum mixing method of Dzung \cite{dzung1971} and the mass average---all three requiring details on other primal flow quantities compared to the area average. Other notions include analyzing radial profiles and using them for engine prognostic and diagnostic efforts. 

\begin{figure}
\centering
\includegraphics[width=0.8\textwidth]{Figures/Fig3.pdf}
\caption{Breakdown of engine temperature measurements.}
\label{fig:measurements}
\end{figure}

But how precise is our averaging process given that we do not approximate the spatial flow field itself? Furthermore,  how do we account for the uncertainties introduced by both individual measurements and any spatial model? As engine measurements shape our understanding of the aerothermodynamics of the gas path, the answers to these questions are of great importance. Moreover, as these measurements (and subsequent inferences) make their way into preliminary design tools and overall uncertainty budgets, inaccurate estimates of both spatial approximations and their averages can have repercussions on new engine programs, measurement and testing practices, and even sub-system-level design.  

In the first part of this two-part paper (see part II in \cite{seshadri2019b}), we develop a framework for studying engine temperature measurements with a more principled, data-centric approach. Specifically, we propose a regression-based model for approximating the spatial flow-field at a given axial plane. To the best of the authors' knowledge, there remains a dearth of publicly available information on this subject; in section~\ref{sec:lit} we discuss prior work done in this area and highlight our contributions. In section~\ref{sec:model} we detail our regression-based model and deploy it on a range of engine data-sets. Finally, in section~\ref{sec:area}, we address the issue of area averaging. 

==> sec-4a.tex <==
\section{An assumed case study}
\label{sec:area}
In section~\ref{sec:lit} we mentioned that owing to the constraints imposed by the Nyquist-Shannon sampling theorem, we cannot recover the amplitudes and phases of all the harmonics using classical fast Fourier transform techniques. We also commented that, although methods based on $l_1$ norm minimization can potentially aid in signal recovery, they require sparsity in the coefficients. In this section, we study two particular aspects of these statements with the objective of recovering the entire spatial temperature profile---not simply the first two harmonics---with sparse measurements. 

In our analysis thus far, we have operated under the premise that we do not know what the \emph{true} spatial variation in temperature is. To expose our methods, and to offer techniques to the wider turbomachinery community, we study an analytically generated temperature profile, shown in Fig.~\ref{fig:assumed_profile}. This profile has an average temperature value of 526.85 K and is comprised of four harmonics $\boldsymbol{\omega}=\left(1, 4, 19, 49 \right)$. 

\subsection{Identifying the harmonics}
Our goal here is apply the regularized least squares approach from Sec.~\ref{sec:model} on this temperature profile to determine whether the approach can capture the two dominant frequencies with only 6 rakes; in some sense serving as a validation of Algorithm 1. 

\begin{figure}
\centering
\includegraphics[scale=0.6]{Figures/Fig14.pdf}
\caption{An assumed temperature profile with four harmonics; the amplitude and phases are varied from hub to casing.}
\label{fig:assumed_profile}
\end{figure}

We study four different sets of virtual rake positions, defined by the values of $\boldsymbol{\theta}$, shown in Table~\ref{table:rakes}. The first is based on the arrangement in Engine A, while the other three are randomly selected such that there is at least one rake in each of the four quadrants. Fig.~\ref{fig:error_assumed} plots the $\varepsilon_{p}^{2}$ (once again on a base-10 logarithm scale) errors using all 6 rakes---i.e., we do not split the data into a testing and training set. It is clear that across all four rake positions, $\boldsymbol{\omega} = \left(1, 4 \right)$ does yield the lowest error; however, there are other frequency pairs that also yield low errors, e.g., $\boldsymbol{\omega} = \left(1, 6 \right)$, $\boldsymbol{\omega} = \left(4, 9 \right)$ and $\boldsymbol{\omega} = \left(6, 9 \right)$, but only for some sets of rake positions. 

\begin{table}
\begin{center}
%\resizebox{\columnwidth}{0.95}{
\caption{Rake positions for the assumed temperature study.}
\begin{tabular}{|c|c|}
  \hline		
 Case & Rake positions (in deg$^\circ$) \\ \hline
 \hline
I & 54, 90, 162, 234, 306, 342 \\
II & 15, 45, 123, 190, 250, 316 \\
III & 60, 114, 180, 250, 310, 351 \\
IV & 0, 75, 150, 220, 250, 320 \\
  \hline  
\end{tabular}
\label{table:rakes}
\end{center}
\end{table}

\begin{figure}
\centering
\includegraphics[scale=0.6]{Figures/Fig16.pdf}
\caption{Values of the error $\varepsilon^{2}$ for four different sets of rake positions.}
\label{fig:error_assumed}
\end{figure}

The temperature profiles associated with $\boldsymbol{\omega} = \left(1, 4 \right)$ are illustrated in Fig.~\ref{fig:final_temps} for the four different rake positions. Although the rake positions are different, the spatial profiles are similar. In fact, even if the rakes were circumferentially equidistant from each other, one can still recover similar patterns to Fig.~\ref{fig:final_temps}.

\begin{figure}
\centering
\includegraphics[scale=0.53]{Figures/Fig15.pdf}
\caption{Temperature profiles for four different rake positions with $\boldsymbol{\omega}=\left(1, 4 \right)$.}
\label{fig:final_temps}
\end{figure}

\subsection{Signal approximation}
In this subsection, we are interested in ascertaining whether we can estimate the amplitudes and phases of all four harmonics given 6 rakes, assuming a priori information on the harmonics is known. This leads to the solution of an undetermined system of equations where $\mA \in \mathbb{R}^{6 \times 9}$. While there are infinitely many solutions to such a linear system, we are interested in the solution that has the lowest $l_2$ norm. Note that this solution strategy is different from the previously discussed L-curve approach, which is typically used on tall or square matrices; our matrix here is fat with more columns than rows. One approach to compute the \emph{minimum norm} solution is given below. Let 
\begin{equation}
\mA \left[\begin{array}{cc}
\mP_{1} & \mP_{2}\end{array}\right] = \left[\begin{array}{cc}
\mQ_{11} & \mQ_{12}\end{array}\right] \left[\begin{array}{cc}
\mR_{11} & \mR_{12}\\
\boldsymbol{0} & 0
\end{array}\right]
\end{equation}
be the pivoted QR factorization\footnote{The pivoted QR factorization is a well-known heuristic for subset selection. See page 276 in Golub and Van Loan \cite{golub2013matrix}} of $\mA$, where $\mP$ is a permutation matrix, $\mQ \in \mathbb{R}^{6 \times 6}$ is an orthogonal matrix and $\mR \in \mathbb{R}^{6 \times 9}$ has the sub-matrix $\mathbf{R}_{11}$ that is upper triangular. These matrices have been partitioned based on the numerical rank of $\mA$, which depends on the rake positions in $\boldsymbol{\theta}$. In this example we use rake positions corresponding to case I, which yields a rank of 5. Thus, $\mR_{11} \in \mathbb{R}^{5 \times 5}$ (and is invertible), $\mP_{1} \in \mathbb{R}^{9 \times 5}$ and $\mQ_{11} \in \mathbb{R}^{6 \times 5}$. The \emph{least norm} solution is then given by
\begin{equation}
\mX = \mP_{1} \mR_{11}^{-1} \mQ_{11}^{T} \mB,
\label{equ:least_norm}
\end{equation}
where as before $\mB \in \mathbb{R}^{6 \times 7}$. Fig. \ref{fig:assumed_profile_slices} plots the circumferential distribution of temperature at measurement points close to the hub, mid-span and casing. The red line in this figure corresponds to the least norm solution (obtained using \eqref{equ:least_norm}), the thick gray line corresponds to the standard least squares approximation with only the first two harmonics, and the black line represents the true temperature distribution.

\begin{figure}
\centering
\includegraphics[width=8.0cm]{Figures/FigX.pdf}
\caption{An assumed temperature profile with four harmonics; the amplitude and phases are varied from hub to casing.}
\label{fig:assumed_profile_slices}
\end{figure}

While the least norm solution does not offer perfect signal recovery, it is able to match the measurements exactly at the measurement locations, and offers an acceptable approximation to the true temperature distribution. It should be noted that this heuristic works even if we alter the amplitudes of the four harmonics---even setting them to be equivalent.

\subsection{A comparison of area averages}
It is worth reiterating our motivation for approximating the full spatial temperature field. First, images such as those shown in Fig.~\ref{fig:final_temps} are useful to understand key engine modes and to identify spatial asymmetries. They are also very important for computing averages.

Recall the discussion in section~\ref{sec:intro} on averaging practices. For the engine measurements considered throughout this paper, we do not have mass-flow rate distributions to compute mass-weighted or momentum-weighted averages. It is not uncommon to area average the temperature measurements and then compute an area-to-mass conversion factor, as shown in Fig. \ref{fig:workflow}. This conversion is usually estimated by CFD on the engine component; a process that in itself has uncertainties well beyond the scope of this work. What we are concerned with here is the way the area average in Fig.~\ref{fig:workflow} is computed. 

\begin{figure}
\centering
\includegraphics[width=8.5cm]{Figures/Fig11.pdf}
\caption{Workflow from thermocouple measurements to a spatial average.}
\label{fig:workflow}
\end{figure}

When using the standard area averaging approach, each measurement is weighted by the sector area coverage associated with its probe (see page 8 in \cite{skiles1980turbine}). Thus, no allowance is made to account for scenarios where the rake positions may capture only the peaks or the troughs of the wave forms. In fact, for the assumed profile considered in this section, the area weighted average technique yields a temperature of 526.20 K. 

For integrating the approximated spatial field, consider the formula in \eqref{equ_expectation}. This can be written as
\begin{align}
\begin{split}
T_{avge} =  & = \frac{1}{\pi\left(r_{o}^{2}-r_{i}^{2}\right)}\int_{r_{i}}^{r_{o}}  \int_{0}^{2 \pi} \vv^{T} \left(r\right) \mU \mX^{T} \va \left(\theta\right)   r dr d\theta \\
& =  \frac{2}{\left(r_{o}^{2}-r_{i}^{2}\right)}\int_{r_{i}}^{r_{o}}  r \vv^{T} \left(r\right) \mU\left[\begin{array}{cc}
\vx_{1}^{T} & \boldsymbol{0}
\end{array}\right] dr
\end{split}
\label{equ:area_new}
\end{align}
where we have used the fact that the harmonic terms in $\va$ (all terms except the first one), when integrated between 0 to $2\pi$, will become zero. Here $\vx_{1}^{T}$ corresponds to the first column of $\mX^{T}$, which comprises of the constant terms of each of the $M$ Fourier expansions. As both approximations in Fig. \ref{fig:assumed_profile_slices}, corresponding to $\boldsymbol{\omega}=(1,4)$ and $\boldsymbol{\omega} = (1,4,19,49)$, are able to obtain the same value of the constant terms, their area averages computed using \eqref{equ:area_new} are equivalent. We report an area average of 525.85 K, which is greater than the area weighted value, but equivalent to the profile average temperature value. Area average temperature comparisons across extracts in Engines A through E---between \eqref{equ:area_new} and the sector weighted area average value---revealed differences between 0.5 and 2 K.
